Plasmon-Phonon Hybridization in Doped Semiconductors from First Principles

Although plasmons and phonons are the collective excitations that govern the low-energy physics of doped semiconductors, their nonadiabatic hybridization and mutual screening have not been studied from first principles. We achieve this goal by transforming the Dyson equation to the frequency-independent dynamical matrix of an equivalent damped oscillator. Calculations on doped GaAs and TiO2 agree well with available Raman data and await immediate experimental confirmation from infrared, neutron, electron-energy-loss, and angle-resolved photoemission spectroscopies.

==> xx.tex <==



==> xy.tex <==


